HREyes: Design, Development, and Evaluation of a Novel Method for AUVs to Communicate Information and Gaze Direction

We present the design, development, and evaluation of HREyes: biomimetic communication devices which use light to communicate information and, for the first time, gaze direction from AUVs to humans. First, we introduce two types of information displays using the HREye devices: active lucemes and ocular lucemes. Active lucemes communicate information explicitly through animations, while ocular lucemes communicate gaze direction implicitly by mimicking human eyes. We present a human study in which our system is compared to the use of an embedded digital display that explicitly communicates information to a diver by displaying text. Our results demonstrate accurate recognition of active lucemes for trained interactants, limited intuitive understanding of these lucemes for untrained interactants, and relatively accurate perception of gaze direction for all interactants. The results on active luceme recognition demonstrate more accurate recognition than previous light-based communication systems for AUVs (albeit with different phrase sets). Additionally, the ocular lucemes we introduce in this work represent the first method for communicating gaze direction from an AUV, a critical aspect of nonverbal communication used in collaborative work. With readily available hardware as well as open-source and easily re-configurable programming, HREyes can be easily integrated into any AUV with the physical space for the devices and used to communicate effectively with divers in any underwater environment with appropriate visibility.

==> fig/active_luceme_accuracy.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/plots/hreye_accuracy_nl.png}
    \caption{Recognition accuracy for active lucemes.}
    \label{fig:active_accuracy}
    \vspace{-5mm}
\end{figure}

==> fig/active_luceme_confusion.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/plots/hreye_confusion.png}
    \caption{Confusion matrix of participant identifications of active lucemes.}
    \label{fig:active_confusion}
    % \vspace{-5mm}
\end{figure}    
    
    

==> fig/active_luceme_operational.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/plots/hreye_opacc_nl.png}
    \caption{Operational recognition accuracy for active lucemes.}
    \label{fig:active_op-acc}
    \vspace{-5mm}
\end{figure}    
    
    

==> fig/system_diagram.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth, trim={0.1cm .9cm 0.1cm 0.2cm},clip]{img/hreye_pcb.png}
    \caption{PCB diagram of an HREye device. \\\textit{(Credit: PCB file Adafruit, PCB diagram Fritzing)}}
    \label{fig:hreye}
    \vspace{-5mm}
\end{figure}    
    
    

==> src/8_acks.tex <==
\section*{Acknowledgments}
The authors wish to thank their colleagues at the Interactive Robotics and Vision lab, particularly Chelsey Edge, Elsa Forberger, Corey Knutson, Demetrious Kutzke, Nyomi Morris, Sakshi Singh, and Jorden Zumberge, who all aided in the administration of the pool study. We also wish to thank our anonymous participants for their participation.

==> src/old_thesis.tex <==
\chapter{Robot-To-Human Communication -- Emitted Light}
\label{r2h:sec:lucemes}

As previously mentioned, light has been proposed as a communication medium for underwater robots~\cite{demarco_underwater_2014}, but not extensively evaluated. 
Light-based communication is utilized as a communication medium for many devices (power indicator lights, turn signals, etc).
Robot-to-human communication using lights is also common, with most robots having at a few indicator lights showing the status of some internal property. 
Further than simple power and system state lights, Baraka et al.~\cite{baraka_enhancing_2016,baraka_mobile_2018} have studied the benefits of using expressive sequences of lights for service robots.
Their programmable light arrays communicated the robot's internal state and planned actions to human interactants to great effect.
Many robot also use lights to indicate affective state, such as Softbank Robotic's Pepper~\cite{noauthor_pepper_nodate} and Nao~\cite{noauthor_nao_nodate} robots as well as Sony's Aibo~\cite{noauthor_sony_nodate} robots.
Song et al.~\cite{song_bioluminescence-inspired_2018} applied similar light arrays to a Roomba, developing light displays which were intended to imply hostility or openness. 
Our work on light-based communication for AUVs as described in the following chapter has developed from simple multi-colored light schemes to a bio-mimetic device with multi-color animations.


\subsection{Definition: Luceme}
\label{r2h:sec:luceme:definition}
Our work on emitted light for AUV communication is focused on the production of \textit{lucemes}, a sequence of light illumination with an associated meaning. 
These sequences include the color, order and duration of illumination, and in some cases the intensity of illumination. 
The word luceme comes from the Latin \textit{luc}, meaning \enquote{light} combined with the Greek \textit{eme}, a unit of linguistic structure.
In previous writing, we have referred to lucemes as \enquote{light sequences}, \enquote{light codes}, or \enquote{LED codes}.
In this document, a luceme will be designated by the symbol \luceme{meaning}, where \enquote{meaning} is parameterized as a simple description of the meaning.


\input{src_tex/2_r2h/fig/hreye/led_system_evoluation}

\section{Baseline Light Communication}
\label{r2h:sec:lucemes:baselines}
Our first attempts at using emitted light as an AUV-to-human communication vector began with the studies described in Sections~\ref{r2h:sec:kinemes:pilot1:design} and~\ref{r2h:sec:kinemes:mds:design}. 
The light systems for these studies (seen in Figure~\ref{r2h:fig:led_evolution:nine} and Figure~\ref{r2h:fig:led_evolution:three}, respectively), were designed to act as a comparison to the RCVM communication described in Section ~\ref{r2h:sec:kinemes}.
The 9-LED version of the system was designed as an attempt to create an encoding from light color and flash rates to semantic meaning, building on the suggestions of Demarco~\cite{demarco_underwater_2014} and Verzijlenberg~\cite{verzijlenberg_swimming_2010}, who both created communication systems utilizing a single-color light's flashes.
This idea was further refined in the 3-LED version, reducing the number of individual LEDs by using full RGB diodes, enabling those three lights to not only produce the red, yellow, and green lights of the 9-LED system, but also blues, purples, and many other colors.
Additionally, further use was made of light \enquote{animation}, with some lucemes indicating direction by illuminating lights in a certain sequence to imply \enquote{left} or \enquote{right}.

\section{Performance of Emitted Light}
\label{r2h:sec:lucemes:performance}
Both the 9-LED and 3-LED system evaluations were described in previous sections, but to summarize: lucemes are a good way of communicating with humans. 
At the highest level of education in RCVM Pilot study I (Section~\ref{r2h:sec:kinemes:pilot1:res-accuracy}, the 9-LED system achieved a recognition accuracy of $60\%$, an operational accuracy of $80\%$, and an average response time of $10$s.
Similarly in the multi-dimensional study, at the ideal viewpoint, the 3-LED system achieved an accuracy of $70.4\%$, an operational accuracy of $58.2\%$, and an average response time of $28.3$ seconds.
In this study however, it was demonstrated that changes in viewpoint had a significant effect on accuracy $F(4, 15.3) = 11.29$, $p < .001$, with accuracy falling to $14.3\%$ at a distance of 8 meters and $13.3\%$ at a 90\degree{} angle.
Taken as a whole, these results show a reasonable recognition accuracy and response time for light-based communication, but a weakness to viewpoint change. 

However, in our more detailed analysis of the performance of different specific lucemes, we found some lucemes to be lower-performing, with recognition accuracy which implies that those lucemes are not intuitive to learn or recall. 
While some issues in luceme recognition could potentially be rectified by redesign, some issues are rooted in the hardware itself.
For the 9-LED system, the light state space could be encoded in nine binary values over time, representing whether each light was on or off.
Spatially, the 9-LED system could be considered as nine points on a line. 
The 3-LED system could be encoded in 9 integer values (a 3-tuple of integers per light, representing red, green, and blue) over time, and spatially represented as 3 points on a line. 
This encoding space was far larger than the system presented in Demarco's case study~\cite{demarco_underwater_2014}, though that system had the benefit of being based on hardware already present in the AUVs in question. 
Nonetheless, our systems suffer from the limitation of their encoding space, both in terms of the sheer amount of information communicable in their state and in terms of the spatial limitations of their structure (how can one indicate motion in the y-axis via a series of points on the x-axis?). 
For this reason, further development of light-based communication of AUVs is necessary.


\section{HREyes: Ocular-Mimicking Emitted Light Devices}
\label{r2h:sec:lucemes:hreye}
To provide AUVs with a more highly communicative and intuitive light-based communication method, we present the HREye, a biomimetic LED device for human-robot interaction. 
HREyes are comprised of 40 individually addressable RGB light emitting diodes arranged in two concentric circles.
Built by daisy-chaining two NeoPixel rings, one of 24 LEDs and one of 16 LEDs, an HREye can be used on its own or synchronously with another. 
In our implementation, the HREyes are controlled using ROS, over a \textit{rosserial} connection to a microcontroller which acts as the LED driver.
We have only integrated HREyes into the LoCO AUV, but the devices are modular and straightforward to add to a system, assuming that the AUV has space for the LED rings. 

\input{src_tex/2_r2h/fig/hreye/active_luceme_table}

\subsection{Design Inspiration}
\label{r2h:sec:lucemes:hreye:design}
When designing the HREye, the goal was to create a light-based communication device capable of displaying complex lucemes, of producing an amount of light useful for illuminating the AUV's environment, and of indicating directions in an intuitive manner. 
In order to enable complex lucemes, we had to increase the number of LEDs from previous systems and arrange them in a structure which enables the creation of complex shapes. 
Next, to be useful for illuminating the scene for an AUV's cameras, the lights need to be placed near the AUV's camera. 
Many participants in previous studies have noted that the cameras of AUVs such as LoCO and Aqua seem to be the \enquote{eyes} of the AUV.
This gave rise to the idea for HREyes: arrange a large number of LEDs around the AUV's camera and mimic the appearance of the human eye. 
This helps to fulfill the final design goal by allowing the HREye to mimic human gaze cues. 

An HREye's state can be represented by 40 3-tuples (red, green, and blue values) across time. 
Each tuple relates to a specific LED on the two rings of the HREye. 
Spatially, an HREye can be considered as 40 points on a two-dimensional plane.
In its programming, the HREye device has four modes: \begin{enumerate*}[a)]
    \item Active Luceme
    \item Ocular Luceme
    \item Passive Display
    \item Functional
\end{enumerate*}.
In functional mode, the HREye device simply acts as a functional light, providing artificial lighting for the AUV at a variety of intensities and color grades.  
Passive mode (which has yet to be implemented), is intended as a way for an AUV to increase visibility of its internal state by reflecting otherwise imperceptible information such as the state of its diver detector by the color and intensity of sections of the device's LEDs. 
These two modes are useful, but not the primary focus of our research. 


\subsection{Active Luceme Design}
\label{r2c:sec:lucemes:hreye:active}
In active mode, the HREye device produces lucemes with specific semantic meaning, similar to the kinemes of RCVM. 
The current luceme versions are shown in Table~\ref{r2h:tab:lucemes:active_luceme_table}. 
These lucemes utilize a color and structure mapping protocol intended to improve recognition accuracy. 
First, for color: yellow relates to directional commands or information, red is connected to problems or danger, blue is mapped to information, and purple is used to reference the AUV itself. 
In terms of structure, there is a shared symbol used for \luceme{Danger} and \luceme{Attention} to indicate time-crucial information, a pulsing illumination used for \luceme{WaitCMD} and \luceme{Malfunction} to indicate a state which requires diver intervention, and a circular animation with one segment of light following another to connect the \luceme{FollowMe} and \luceme{FollowYou} lucemes. 

\input{src_tex/2_r2h/fig/hreye/ocular_luceme_table}

\subsection{Ocular Luceme Design}
\label{r2c:sec:lucemes:hreye:ocular}
Ocular lucemes are much more uniform than their active counterparts. 
All ocular lucemes follow the same structure: the inner ring is illuminated in pink (recalling the iris), with the outer ring illuminated in white (recalling the sclera). 
The color pink was selected as it had not been used in many lucemes, was similar to the color used to reference the robot, and would be highly noticeable in the water. 
The ocular lucemes created (depicted in Table~\ref{r2h:tab:lucemes:ocular_luceme_table}) include a steady state luceme, lucemes for blinking, squinting, and widening eyes, and a set of gaze cues with 30\degree granularity.
The gaze lucemes are the only ones which have been evaluated in human studies, but the other lucemes were designed mostly to communicate affect and thus require a different form of evaluation.


\section{HREye Evaluation Study}
\label{r2h:sec:lucemes:hreye_eval}
With our HREye devices design, built, and programmed with active and ocular lucemes, we must turn our attention to evaluating the HREye system. 
In the following sections we describe our initial HREye evaluation study, which tests the recognition accuracy of active and ocular lucemes via a human study in a pool.
The study described in this section was approved as human research by the University of Minnesota's institutional review board (reference number: 00015327) and determine to be exempt from continuing review.

\subsection{Study Design}
\label{r2h:sec:lucemes:hreye_eval:study}
Our study of HREye performance is based around recording the results of human recognition of HREye lucemes in a pool environment.
In short, we recruited participants, trained them to a point of competency in the use of the HREye system several days beforehand, then had them identify active lucemes as produced on the LoCO-AUV's HREyes, in a pool.
The results from this pool evaluation serve to demonstrate the performance of the active lucemes of HREye, when being shown to a trained interactant. 
Following this, we also asked each participant to identify the gaze direction of the ocular luceme gaze cues, a system on which they had not been trained.
To provide a point of comparison to the HREye-trained participants, we will also collect data on human recognition of information passing from the AUV's OLED display, though this has not yet been completed. 
As the OLED display condition will be very quick for participants to test, we also plan to have the participants of that condition evaluate the HREye active lucemes with no training, to gather data on the intuitiveness of the active lucemes.


\subsection{Administration}
\label{r2h:sec:lucemes:hreye_eval:administration}
A total of 8 participants were recruited for the study via student email lists.
After collecting participant consent to the study practices and administering a short demographic survey, participants were trained to use the HREye communication devices. 
This was done by displaying a video of 4-5 lucemes with their meanings displayed on screen, then testing the participants on luceme recognition. 
Once this had been done for all lucemes (three batches of 4-5 lucemes), a final competency test was administered, asking participants to identify each luceme. 
Participants who correctly recognized at least 12 out of the 16 lucemes passed the competency test, and were scheduled for a pool evaluation slot.
These pool evaluation times occurred no more than 7 days from initial training.

In the pool evaluation portion of the survey, participants were given a quick refresher of the list of luceme meanings.
Following this, participants entered the pool a few feet from the LoCO AUV, then were shown the lucemes of the HREye system in a randomized order. 
For each luceme, the participant dove under the water, observed the luceme display, then surface and verbally indicated what they thought the luceme meant.
The time from the beginning of the luceme until the beginning of the participant's answer was recorded, along with the participant's confidence in their answer ($0$ - $10$). 
Once all active lucemes had been tested, participants were asked to continue the same process while being shown ocular lucemes for gaze indication (which they had not been previously shown). 
Participants were told to report the meaning of the ocular lucemes in terms of directions (left, right, up, down) or analogue clock time (1 o'clock, 6 o'clock).
Following their completion of the pool evaluation, participants were asked to complete a quick debrief survey which consisted of a modified Godspeed~\cite{bartneck_measurement_2009, weiss_meta_2015} questionnaire and a set of NASA Task-Load Index (TLX)~\cite{hart_development_1988,noyes_self-analysis_2007} questionnaires, one for active luceme recognition and one for ocular recognition.
The Godspeed questionnaire measures participant opinion on the AUV they were shown, while the NASA TLX questionnaires measure the amount of mental, physical and temporal demand that the luceme recognition placed on participants.
With the debrief survey completed, participants were given a gift card with a value of $10$ USD. 

\subsection{Analysis}
\label{r2h:sec:lucemes:hreye_eval:analysis}
With the data from our demographic survey, pool evaluation sessions, and debrief surveys collected, we turned to data analysis. 
The demographic and debrief survey data can be analyzed without further processing, but the pool evaluation session data required some further work. 
Because participants had answered questions about luceme meanings freely, their response had to be transformed into a usable format.
For active lucemes, three raters were given a list of active lucemes shown to participants, matched with the meanings participants reported. 
The three raters then scored each pair with a correctness score between $0$ and $100$.
An inter-rater reliability analysis using Fleiss' Kappa~\cite{fleiss_measuring_1971} was performed to evaluate consistency between raters. 
The inter-rater reliability was found to be $\kappa = 0.683$, which is generally taken to mean that there is substantial agreement between raters~\cite{landis_measurement_1977}. 
Since rater consistency is high, we simply averaged the rater's scores with no weighting to create the final accuracy score for each active luceme.
In the case of the ocular luceme responses, raters were not needed.
Since answers were almost all given in terms of directions or analogue clock time, they can be simply translated into the angle of the gaze cue in degrees. 
With these two processing steps completed, we can continue to final analysis of the performance of both active and ocular lucemes.
We utilize the same metrics used in our RCVM studies: accuracy (0-100 recognition rate), operational accuracy (0-100, same as accuracy, but only considering high accuracy), confidence (0-10, participant reported), and time to answer (time between luceme beginning and participant answer).


\subsection{Results -- Demographics}
\label{r2h:sec:lucemes:hreye_eval:demographics}
Our study population was comprised of 8 people.
Seven of these were students, the other was employed full-time.
When asked to self-identify their gender, five identified as male, two as female, and one identified as non-binary.
All but one were in the age range of 18-24, the remaining participant was between 25-34.
When asked about their country of origin, all but one participant responded that they were from the United States, and all participants had been in the US for at least five years. 
Participants were asked about their experience with robotics, scuba diving, and sign language.
Half indicated that they had experience with robots, half indicated some level of scuba diving experience, and half indicated a familiarity with some kind of sign language.
Lastly, participants were asked about their vision.
Fifty percent of participants self-reported nearsightedness and none reported colorblindness, which was confirmed by a self-administered Ishihara test~\cite{birch_efficiency_1997}.

\input{src_tex/2_r2h/fig/hreye/active_luceme_accuracy}
\input{src_tex/2_r2h/fig/hreye/active_luceme_operational}

\subsection{Results -- Active Lucemes}
\label{r2h:sec:lucemes:hreye_eval:active}
In our pool testing, participants identify active lucemes with a high overall accuracy of $80\%$.
As shown in Figure~\ref{r2h:fig:hreye:active_accuracy}, the directional lucemes all achieve high accuracy (with the exception of \luceme{Go left}, with \luceme{WhichWay} achieving a perfect recognition accuracy.
In terms of operational accuracy, shown in Figure~\ref{r2h:fig:hreye:active_op-acc}, participants achieve an even higher rate of $90\%$, with a number of lucemes even hitting $100\%$ operational accuracy.
Average participant time-to-answer is $10.6$ seconds, with the \luceme{Attention} and \luceme{Malfunction} being two of the longer response times. 
This is consistent with the relatively lower accuracy of these lucemes, indicating some confusion on those kinemes, which be more clearly seen in Figure~\ref{r2h:fig:hreye:active_confusion}. 
Note that in the confusion matrix, it is obvious that participants are confusing \luceme{FollowMe} and \luceme{FollowYou}, which have similar animations with the only differnce being the color of the inner ring.
Similarly, lucemes which heavily feature the color red, such as \luceme{Negative}, \luceme{Danger}, and \luceme{Malfunction} are confused for one another.
This suggests that further separating lucemes in color space and ensuring that lucemes with similar animations have large differences in color may improve recognition accuracy by reducing confusions.
This will be discussed further in Chapter~\ref{future_chapter}, Section~\ref{future:sec:exante}: Ex Ante Interaction Phrase Analysis.


\input{src_tex/2_r2h/fig/hreye/active_luceme_confusion}

\input{src_tex/2_r2h/fig/hreye/ocular_luceme_accuracy}

\subsection{Results -- Ocular Lucemes}
\label{r2h:sec:lucemes:hreye_eval:opinion}
In our pool testing, participants correctly identified gaze cues with high accuracy. 
While some participants had confusion about the gaze cues initially, all participants realized the key idea: the purple center was the pupil, the motion of gaze lucemes was meant to indicate motion of the pupil in a direction.
Overall, participants interpreted ocular lucemes with an average error of 24\degree, as visualized in Figure~\ref{r2h:fig:hreye:gaze}.
Some of this angle error may have been due to the fact that in one session, the HREye in the LoCO AUV's right enclosure began to slip and rotate, rotating almost 45\degree before the issue was detected. 
Remaining participants in that session were only shown gaze cues on the left HREye, and the issue was rectified with proper mounting before the following session.
Nonetheless, even with this confounding issue, interactants seem to be able to intuitively understand the gaze direction of an AUV using the HREye ocular lucemes. 
It remains to be seen how well this translates to grounding tasks in underwater environments, however, as post-study interviews with some participants suggested that participants did not feel the robot was actually looking in the directions it was indicating. 

\section{Conclusion and Future Directions}
Our preliminary study of the HREye device demonstrated its effectiveness as a method of transmitting information using emitted light. 
Not only did our study demonstrate a recognition accuracy of 80\% for trained participants in active communication mode, we also showed that participants understood gaze cues with an average directional error of $24$\degree.
In the future, we plan to collect more data on active luceme intuitiveness and comparison to other data by collecting data on a baseline system (a digital display), and having those participants attempt to identify active lucemes with no training on the HREye system.
Additionally, we hope to determine how effective gaze cues can be in actual interactions by performing gaze grounding experiments.
